A Maude Implementation of Rewritable Petri Nets: a Feasible Model for Dynamically Reconfigurable Systems

Petri Nets (PN) are a central, theoretically sound model for concurrent or distributed systems but, at least in their classical definition, not expressive enough to represent dynamic reconfiguration capabilities. On the other side, Rewriting Logic has proved to be a natural semantic framework for several formal models of concurrent/distributed systems. We propose a compact, efficient Maude formalization of dynamically reconfigurable PT nets (with inhibitor arcs), using as a running example the specification of a simple, fault-tolerant manufacturing system. We discuss the advantages of such a combined approach, as well as some concerns that it raises.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{M. Gleirscher, J.v.d. Pol, J. Woodcock (Eds.):\\First Workshop on Applicable Formal Methods (AppFM 2021).\\
EPTCS 349, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.349.3}{10.4204/EPTCS.349.3}}

